Towards Resilient and Sustainable Global Industrial Systems: An Evolutionary-Based Approach

This paper presents a new complex optimization problem in the field of automatic design of advanced industrial systems and proposes a hybrid optimization approach to solve the problem. The problem is multi-objective as it aims at finding solutions that minimize CO2 emissions, transportation time, and costs. The optimization approach combines an evolutionary algorithm and classical mathematical programming to design resilient and sustainable global manufacturing networks. Further, it makes use of the OWL ontology for data consistency and constraint management. The experimental validation demonstrates the effectiveness of the approach in both single and double sourcing scenarios. The proposed methodology, in general, can be applied to any industry case with complex manufacturing and supply chain challenges.

==> conclusions.tex <==
\section{Conclusions and Further Steps}
\label{sec:conclusions}

This report describes the results of a research work done for an European aerospace manufacturer for the optimization the industrial system. The solution of the research was adapted and verified on a given set of input data. The evolutionary algorithm is able to construct the industrial system following the given pre-defined constraints.

Furthermore, the solution for additional tasks, which were not involved within the EA solution, was proposed and implemented as the second phase of the optimization. The successfully covered/solved tasks include:
\begin{itemize}
    \item 
    Create a graph of flows within the supply chain (industrial system formed by the first phase)
    \item 
    Exploitation of warehouses
    \item 
    Distribution of demands and required time across the supply chain based on shares between sites
    \item 
    Single and mixed batching of the parts
\end{itemize}

 However, we were not able to complete tests of the implemented approach due to inconsistencies in input data together with outcomes from the first phase regarding transportation means. In other words, the suitable transportation means was not possible to determine for all of the connections between graph nodes (sites, warehouses); for example, a produced part has to be delivered from a close harbour to the destination (where the suitable transportation may be solved using, e.g., RoRo ship), however, it is not possible to transport the part from the site to the harbour because it does not fit into any available transport mean/container. This obstacle should be overcome by refining the input data, by adding more constraints to the first phase of optimization, or by both of them.

The further steps for improving the presented solution include:
\begin{itemize}
    \item We will consider using a simulation-based approach to solve the \phaseII\ task. This appears to be a suitable approach, especially when the minimal lead time requirement, mixed batching strategies, and warehouses come into play. We have experience with a similar project where we solved the facility layout optimization problem by means of an evolutionary algorithm. There, we used a simulator as an evaluator of candidate plant layouts. For each candidate plant layout, a virtual twin was created in the simulator and tested for a period of time to collect sufficient data to assess the plant layout performance. This way, multiple optimization criteria values can be gathered and used to guide the evolutionary algorithm towards well-performing layouts. 
    \item We will - LP, minimum-cost flow goes here
    \item We will use the \phaseII\ optimization techniques already within the evolutionary algorithm to calculate the quality of generated candidate solutions. This will make the EA solution more robust as the \phaseII\ optimization techniques provide more accurate, reliable, and realistic estimates of the expected industrial system architecture performance.
    \item We will implement a multi-objective EA to simultaneously optimize multiple criteria (minimize recurring transportation costs, minimize CO$_2$ emissions, minimize total transportation distance, etc.). Evolutionary algorithms are particularly suitable for solving tasks of this type with possibly contradictory optimization objectives and objectives whose values differ by orders of magnitude. In such a case, it is hard to use approaches based, for example, on a weighted sum of individual objectives.
\end{itemize}

==> introduction.tex <==
\section{Introduction}
\label{sec:introduction}

This paper presents the results of research work performed at a large European aircraft manufacturer that has focused on the capabilities development and verification for the design of novel, disruptive manufacturing systems for future aircraft programs. 

\jiri{adopted from: Industrial System Constraints for Optimisation Challenge new.pdf}{In today’s globalized world, the production of commercial aircraft has become a complex and highly distributed process. With production sites scattered across different countries, manufacturers rely on a vast network of internal facilities and suppliers.

The production of an aircraft requires the transportation of large parts such as wings, engines, or fuselage sections between different production sites. To transport these large parts, special transportation means such as oversized road transporters, special aircraft freighters like \andi{\st{the Beluga} transportation aircraft} and special ships have to be used.

The transportation of these large parts is not only costly, but also leads to high CO$_2$ emissions. Therefore, finding a routing in the network minimizing logistics-related costs and CO$_2$ emissions is crucial.

An industrial system data model is used to provide building blocks for creating industrial system architectures automatically. The purpose of such an architecture is to create a final product out of its parts and subassemblies; in this case a single aisle aircraft.
%
The data model itself contains structures to represent all the concepts, relations and meta data to evaluate different architectures
through a set of KPIs defined by the aircraft manufacturer.

The scope of the model is at a macro economic scale. This means that it is concerned with where the different parts of the aircraft are being manufactured, and how they are transported between different production locations all over the world.
This includes batching - loading multiple parts into one transport mean (if the parts are different from one another it is called mixed batching) - and sourcing the same part from different sources to increase the resilience of the industrial system. Usually this means from two source in two different countries (double sourcing).

The instantiated data model contains all possibilities for all valid variants of the industrial system. The data already eliminates some invalid variants such as parts transported on invalid transport means. However, several other constraints need to be taken into account such as the workshare between different countries.
}

This paper focuses on the optimization of the industrial system architecture, in particular the topology of production locations, sourcing strategies, and transport connections within these production networks. 
%
The optimization process is split into two phases. 

The first phase, \phaseI, uses an evolutionary algorithm (EA) to create an industrial system architecture based on predefined constraints. This architecture defines the supply chain regarding producers and consumers of all parts within the industrial system and production shares between producers of the same part.

The second phase, \phaseII, represents transportation optimization together with batching optimization. \todo[inline]{VJ: 1-2 sentences about the second phase to be added}

The main contributions of this paper are:
\begin{itemize}
    \item A new complex optimization problem for automatically designing industrial system architectures has been formulated. It involves challenges that every manufacturing company with a large network of manufacturing facilities and suppliers scattered across different countries faces today.
    \item An approach combining an evolutionary algorithm, formal mathematical programming methods, and an ontology-based data model was designed to solve the proposed optimization problem.
    \item \todo[inline]{TBD: Contribution(s) related to the ontology-based industrial system data model}
    \item \todo[inline]{Can we make the dataset publicly available?}
\end{itemize}

This paper is organized as follows: First, a detailed problem description is provided in Section~\ref{sec:problem_definition}. Next, the first and second optimization phases are described in Section~\ref{sec:phaseI} and Section~\ref{sec:phaseII}. Experiments and their discussion are presented in Section~\ref{sec:experiments}. Finaly, Section~\ref{sec:conclusions} concludes the paper.


==> problem_definition.tex <==
\section{Problem Definition}
\label{sec:problem_definition}

% The task to solve is similar to the problem from former research work as described in ~\cite{airbus2023a}. However, the current problem is extended by several new constructs and features.
\jiri{}{This section provides a formal definition of the problem addressed in this work. 
% The problem involves the design of an optimal industrial system architecture with respect to multiple optimization objectives related to the feasibility of the architecture and its transportation costs, subject to a number of constraints.
The problem involves the design of an optimal industrial system architecture with respect to the overall transportation costs, subject to a number of constraints.

Following is a list of entities that appear in the problem definition:
\begin{itemize}
    \item Production graph \prodgraph\ -- the manufacturing process of the final product can be formally described by a tree, where the root node represents the \textit{final product}, the leaf nodes are atomic, further indivisible, parts of the product, and the internal nodes represent composite parts assembled from the parts that are at the input to the internal node.
    \item \parts\ -- a set of $M$ parts, $\{p_1, \dots, p_M\}$, present in the production graph \prodgraph, i.e., the final product, all composite parts, and all atomic parts.
    \item \psites\ -- a set of production site locations; in each location, one or more production plants are operated.
    \item \countries\ -- a set of countries where the production sites are located.
    \item \pplants\ -- a set of production plants (factories), where each production plant is assigned to a particular production site $l\in$\,\psites\ in one specific country $c\in$\,\countries. Each plant can produce one or more types of parts. The set of parts available for plant $f$ is denoted as $P^f \subset$\,\parts.
    \item \suppliers\ -- a set of suppliers which can be involved in producing the final product. A supplier operates production plants at several production sites (one plant at a site) in various countries.
    \item \punits\ -- a set of production units \punits\, where each production unit is a unique pair of a particular supplier $s\in$\,\suppliers\ and one of its production plants $f\in$\,\pplants.
    \item \punitsp\ --  a subset of production units \punitsp\,$\subset$\,\punits\ such that each $u\in$\,\punitsp\ can produce the particular part $p\in$\,\parts.
    \item \punitss\ --  a subset of production units \punitss\,$\subset$\,\punits\ that belong to the supplier $s\in$\,\suppliers.
    \item \punitsc\ --  a subset of production units \punitsc\,$\subset$\,\punits\ that are located in the country $c\in$\,\countries.
    \item \warehouses\ -- a set of warehouses that serve as storage for input/output parts for/from several production plants. 
    \item \warehousesu\ -- a subset of warehouses \warehousesu\,$\subset$\,\warehouses\ that are available to the production unit $u\in$\,\punits. 
    \item \va\ -- a value-added \va\ is a real number from the interval (0, 1) that represents the ratio of the value of the part $p\in$\,\parts\ to the total value of the final product.
    \item \vac\ -- a value-added \vac\ is a real number from the interval (0, 1) that represents the actual value-added allocated to the country $c\in$\,\countries\ calculated as the ratio of the sum of values of all parts produced in production units $u\in$\,\punitsc\ to the total value of the final product.
    \item \vas\ -- a value-added \vas\ is a real number from the interval (0, 1) that represents the actual value-added allocated to the supplier $s\in$\,\suppliers\ calculated as the ratio of the sum of values of all parts produced in production units $u\in$\,\punitss\ to the total value of the final product.
    \item \vacmin, \vacmax\ -- required minimum and maximum boundaries on the value-added allocated to the country $c\in$\,\countries. 
    \item \vasmin, \vasmax\ -- required minimum and maximum boundaries on the value-added allocated to the supplier $s\in$\,\suppliers. 
    \item \vaumax\ -- the maximum added-value allowed for the production unit $u\in$\,\punits.   

    \item \trmeans\ -- a set of possible means of transportation that can be used to transport the parts. Each type of transportation $t\in$\,\trmeans\ has specified its CO$_2$ emission \tremission, speed \trspeed, and maximum load volume \trload. 

    % --- Transportation meta-graph
    \item \trmgraph$(\mathcal{N},\mathcal{E})$ -- a transportation meta-graph is a directed graph in which all possible instances of the industrial system can be represented. Its nodes, $\mathcal{N}$, comprise all production units and all available warehouses, i.e., $\mathcal{N}=U \cup W$. 

    The edges in the set $\mathcal{E}$ represent transportation links used to carry a load from the source node to the destination node, i.e., an edge is an oriented link $(u,v)$ where $u,v \in \mathcal{N}$.
    Each edge $\varepsilon \in \mathcal{E}$ can only choose its transportation type $\tau^\varepsilon$ from the set of possible transportation types $T^{\varepsilon} \subset T$ available for the edge. 
    The chosen transportation type determines the edge's length $l^\varepsilon$.
    Further, each edge has its batching size $b^\varepsilon$, which is the number of parts transported in a single shipment along the edge.
    Here, we consider a single-product batching consisting of one or more pieces of the same part. 
    % The part size and the maximum possible load volume of the selected transportation type \trload\ determine the maximum possible value of $b^\varepsilon$.

    % Every shortest path between two nodes $u_1,u_2\in$\,\punits\ in the \trmgraph\ must be either of the type $u_1 \rightarrow u_2$ or the type $u_1 \rightarrow w \rightarrow u_2$, where $w\in$\,\warehouses. In the latter case, the following must hold $w\in W^{u_1}\cap W^{u_2}$.

    % --- Particular transportation graph
    \item \trgraph$(N,E)$ -- a directed graph as a sub-graph of the transportation meta-graph representing a particular industrial system designed to produce the final product. Its nodes $N$ and edges $E$ are a subset of $\mathcal{N}$ and $\mathcal{E}$, respectively. 
    Each edge $e\in E$ has already assigned its particular type of transportation that determines its length $l^e$. It has also specified its batching size $b^e$.
    Finally, a specific part is assigned to every end node $u \in U$ in each edge. The part is chosen from the parts produced by the respective production unit. 
    
    % \item \shipments\ -- a set of all shipments carried out along the edges 
    % The particular selection of the transportation type determines its length $l^\varepsilon$ and the batching size $b^\varepsilon$, which is the number of parts transported in a single shipment. 
    % Here, we consider a single product batching consisting of one or more pieces of the same part. The part size and the maximum load's volume of the selected transportation type \trload\ determine the maximum possible value of $b^\varepsilon$.

    Figure~\ref{fig:transportLinksDist} illustrates the most important components of the transportation graph.
    
\end{itemize}
}
    
% New concepts (with respect to former work) for which the former solution had to be adapted are as follows: 
% \begin{itemize}
%     \item 
%     Parts/Products Batching - parts are transported using various containers/transport means. The batch size is dependent on the part size as well as the type of container. The type of transportation influences the costs as well as transportation time. Furthermore, there are two different batching strategies - single or mixed (where different types of parts are transported together).
%     \item
%     Warehouses - nodes of transportation net with predefined capacity where various parts can be stored and subsequently dispatched for following processing. Obviously, mixed batches may be formed here and thus save costs during long-distance transportation instead of separated single-batch direct transportation between producer production resource and consumer production resource.
% \end{itemize}


%--------------------------------------------------------------------------------------------------------
\subsection{Constraints}
\label{sec:constraints}

The constraints imposed on a valid solution used in this study are defined below. 
%
\begin{itemize}
    \item \textbf{Constraint\,1} -- a part shall only be manufactured by a production unit with the manufacturing capability for said part.
    \item \textbf{Constraint\,2} -- in the case of \textit{double sourcing}, each part has to be produced in two different production units while splitting the whole production of the part between the production units in the ratio $a$~:~$(1-a)$ where $a\in(0,1)$. Moreover, the two production units shall be located in two different countries if applicable. Note that some parts can be produced only in production units where all of them are located in the same country. In such a case, this constraint is not enforced.
    \item \textbf{Constraint\,3} -- in the case of double sourcing, the split between each production unit for the same part shall be between 20\% to 80\%. The sum of the split shall be 100\%.
    \item \textbf{Constraint\,4} -- the value added by the country $c$ is less than or equal to \vacmax\ for all $c\in$\,\countries.
    \item \textbf{Constraint\,5} -- the value added by the supplier $s$ is less than or equal to \vasmax\ for all $s\in$\,\suppliers.
    \item \textbf{Constraint\,6} -- the value added by the production unit $u$ is less than or equal to \vaumax\ for all $u\in$\,\punits.
\jiri{}{
    \item \textbf{Constraint\,7} -- every shortest path between two nodes $u_1,u_2\in$\,\punits\ in the transportation graph \trgraph$(N,E)$ must have one of the following structures
    \begin{enumerate}
        \item $u_1 \rightarrow u_2$,
        \item $u_1 \rightarrow w \rightarrow u_2$,
    \end{enumerate}
    where $w\in W^{u_1}\cap W^{u_2}$, i.e., the warehouse $w$ is common to both production units $u_1$ and $u_2$.
    \item \textbf{Constraint\,8} -- the batching size $b^e$ assigned to an edge $e$ of the graph \trgraph$(N,E)$ can not be larger than the maximum possible value, which is determined by the maximum load's volume \trload\ of the transportation type assigned to the edge and the size of the part transported along the edge.
    % the particular selection of the transportation type determines its length $l^\varepsilon$ and the batching size $b^\varepsilon$, which is the number of parts transported in a single shipment. 
    % Here, we consider a single product batching consisting of one or more pieces of the same part. The part size and the maximum load's volume of the selected transportation type \trload\ determine the maximum possible value of $b^\varepsilon$.
}    
\end{itemize}

% Moreover, some adjustments to the constraints were made in order to be able to deliver a working prototype of the industrial system generator given the current data, see Section~\ref{sec:phaseI}.
%
% We had to adjust some of the constraints to be able to test our EA tool with the given data as follows:
% \begin{itemize}
%     \item \textbf{Constraint\,3} had to be relaxed in special cases since there are parts for which all of the available \textit{ProductionLocations} are located in the same country.\\
%     Examples: 
%     \begin{itemize}
%         \item \textbf{section 1} can only be produced in France \{St. Nazaire, Toulouse, Nantes\} 
%         \item \textbf{wing left} and {wing right} can only be produced in United Kingdom \{Broughton, Belfast\}
%     \end{itemize}

%     \item \textbf{Constraint\,6} is defined as a soft constraint: ``\textit{the value added by some Supplier shall be optimized towards a target value}''. We replaced it with the following hard constraint definition: ``\textit{the value added by some Supplier shall not exceed a maximum value \vasmax}''. This value is an input parameter for the model.
    
%     \item Similarly, we adjusted a definition of \textbf{Constraint\,7} into the hard constraint one: ``\textit{the value added by some ProductionLocation shall not exceed a maximum value \valmax}''. Again, this value is an input parameter for the model.
    
%     \item Double-sourcing cannot be applied to FAL production units since they require part \textbf{s123456\,full\,fuselage} as an input, which is however too large to be transported. To cope with this fact, we slightly modified the production graph so that we eliminated a step with the production of part \textbf{s123456\,full\,fuselage}. Instead, its three input parts \textbf{section~1}, \textbf{section~56}, and \textbf{section~234} are used directly as the input of \textbf{single aisle aircraft}.
% \end{itemize}

Some constraints are relevant only for \phaseI\ and \phaseII, respectively; see below in Section~\ref{sec:phaseI} and Section~\ref{sec:phaseII}. 


%--------------------------------------------------------------------------------------------------------
\subsection{Optimization objectives}
\label{sec:objectives}

\jiri{}{
When designing the optimal industrial system, we consider the following optimization objectives:
\begin{itemize}
    \item Minimize the total amount of CO$_2$ generated while using the \trgraph\ to produce $K$ pieces of the final product. 
    Formally, this objective is defined as
    \begin{equation*}
        \operatorname*{arg\,min}_{G^T(E,N) \in \mathcal{G}} f_1(G^T(E,N))=\sum_{e\in E} n_e * l^e * \tau^e_c
    \end{equation*}
    where $n_e$ is the number of rides carried out along the edge $e$ of the length $l^e$ while using its assigned transportation type $\tau^e$ and emitting $\tau^e_c$ grams of CO$_2$ per kilometer.
    
    \item Minimize the total transportation time spent while using the \trgraph\ to produce $K$ pieces of the final product.
    Formally, this objective is defined as
    \begin{equation*}
        \operatorname*{arg\,min}_{G^T \in \mathcal{G}} f_2(G^T(E,N))=\sum_{e\in E} n_e * \frac{l^e}{\tau^e_s}
    \end{equation*}
    where $n_e$ is the number of rides carried out along the edge $e$ of the length $l^e$ km using the transportation type $\tau^e$ with the speed of $\tau^e_s$ km/hour.
\end{itemize}
}


%------------------------------------------------------------------------------------------------------
\subsection{Constraint optimization problems solved}
\label{sec:opt_problem}

\jiri{}{
In this work, we define the following constraint optimization problems:
\begin{enumerate}
    \item Find the transportation graph $G^T(E,N)$ such that the objective $f_1()$ is minimized subject to all constraints defined above.
    \item Find the transportation graph $G^T(E,N)$ such that the objective $f_2()$ is minimized subject to all constraints defined above.
    \item Find the transportation graph $G^T(E,N)$ such that both objectives $f_1()$ and $f_2()$ are minimized simultaneously subject to all constraints defined above.
\end{enumerate}

% The first two variants are single-objective optimization problems, while the third one is a bi-objective optimization problem. 
In all three cases, the problem faces manifold challenges. Finding the optimal transportation graph requires choosing its optimal topology, optimally assigning parts to production units, and optimally choosing transportation link attributes (transportation type and batching size).
}
